EtiCor++: Towards Understanding Etiquettical Bias in LLMs

In recent years, researchers have started analyzing the cultural sensitivity of LLMs. In this respect, Etiquettes have been an active area of research. Etiquettes are region-specific and are an essential part of the culture of a region; hence, it is imperative to make LLMs sensitive to etiquettes. However, there needs to be more resources in evaluating LLMs for their understanding and bias with regard to etiquettes. In this resource paper, we introduce EtiCor++, a corpus of etiquettes worldwide. We introduce different tasks for evaluating LLMs for knowledge about etiquettes across various regions. Further, we introduce various metrics for measuring bias in LLMs. Extensive experimentation with LLMs shows inherent bias towards certain regions.

==> sections/bias-metrics-ideas.tex <==
\section*{Bias Metrics Ideas} \label{sec:bias_metric}



==> sections/bias-mitigation.tex <==
\vspace{-3mm}
% \section{Checking \taskname} \label{sec:method}
\section{Bias Mitigation Methods}\label{sec:bias_mitigation}
% \vspace{-3mm}
\subsection{DPO Motivation}We propose to use DPO as one of the methods to mitigate the bias exhibited by the model. The reason we choose DPO is because while conducting the experiments, we can clearly see the preference of the biased models for etiquettes some particular regions, mainly Europe, be it acceptability of the etiquettes, preference for etiquettes or alignment with etiquettes. We hypothesise that by preparing a DPO dataset and aligning the model with the correct values of each region, the models will learn to accept, prefer and align with the correct etiquettes of every region. Following the work of \cite{DBLP:conf/acl/Allam24} we build a DPO dataset from \corpusname.
\subsubsection{DPO dataset preparation}
We create a DPO dataset from \corpusname\. We want to create create chosen and rejected responses for each region, for that we iterate over each data point ($p$) of a region ($r$) and find similar sentences over a threshold (0.55) in datasets of other regions (to find sentences about similar concepts). Each similar sentence is a pair ($p$ and the found sentence). Now this list of conceptually similar sentence pairs is going to be filtered if they are entailing or contradicting each other. This is done by performing a Natural Language Inference task using the \textit{facebook/bart-large-mnli} model. The contradicting pairs become a chosen and rejected pair for $r$ and hence a DPO dataset is created for reducing bias.
\begin{tcolorbox}[width=\columnwidth,colback=gray!10,colframe=black,sharp corners]
    PROMPT: You are an expert in cultural etiquettes across various countries. You will be given a region and a topic. You have to provide me with an eitquette regarding the topic in the region. \\ \\
    In the context of [group], Etiquette in [region1] is: \\ \\
    CHOSEN: '[chosen etiquette]'\\ \\
    REJECTED: '[rejected etiquette]'
\end{tcolorbox}

\subsection{Bias Mitigation through Bias Neuron Elimination}


==> sections/corpus-sources.tex <==
\section{Corpus Sources} \label{app:corpus-source}
Websites used for scrapping Etiquette's for different regions are as follows:

\begin{itemize}
  \item \textbf{Indian Culture: Do's and Don'ts} \\
  \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-do-s-and-don-ts#indian-culture-do-s-and-don-ts}
  
  \item \textbf{Indian and Western Values} \\
  \url{https://www.studocu.com/in/document/sree-sankaracharya-university-of-sanskrit/social-work-in-education/indian-and-western-values/31773443}
  
  \item \textbf{Which is the best culture: Indian or Western? (Quora)} \\
  \url{https://www.quora.com/Which-is-the-best-culture-Indian\\-or-Western}
  
  \item \textbf{Indian Culture: Etiquette} \\
  \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-etiquette#indian-culture-etiquette}
  
  \item \textbf{Indian Culture: Core Concepts} \\
  \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-core-concepts#indian-culture-core-concepts}
  
  \item \textbf{Indian Society} \\
  \url{https://indianchild.com/indian_society.htm}
  
  \item \textbf{Indian Etiquette} \\
  \url{https://www.a-to-z-of-manners-and-etiquette.com/indian-etiquette.html}
  
  \item \textbf{Indian Culture: References} \\
  \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-references#indian-culture-references}
  
  \item \textbf{Indian People and Life} \\
  \url{https://factsanddetails.com/india/People_and_Life/sub7_3d/entry-4174.html}
  
  \item \textbf{Difference Between Indian Culture and Western Culture (Ask Any Difference)} \\
  \url{https://askanydifference.com/difference-between-indian-\\culture-and-western-culture/}
  
  \item \textbf{Indian Culture Compared to Japanese Culture} \\
  \url{https://smrutiprakashcom.wordpress.com/#:~:text=Indian%20culture%20compared%20to%20Japanese,culture%20primarily%20focuses%20on%20formality.}
  
  \item \textbf{Work Culture in Japan Compared to India (Quora)} \\
  \url{https://www.quora.com/How-is-the-work-culture-in-Japan-\\in-comparison-to-India}
  
  \item \textbf{Indians in Japan: Jugaad} \\
  \url{https://globisinsights.com/purpose/dei/indians-in-japan-jugaad/}
  
  \item \textbf{Japan v/s India: The Way Business is Run} \\
  \url{https://blog.clrskills.com/japan-v-s-india-the-way-business-is-run/}
  
  \item \textbf{Japan's Unique and Distinctive Work Culture} \\
  \url{https://corporatecitizen.in/v6-Issue8/work-culture-japans-unique-and-\\distinctive-work-culture.html}
  
  \item \textbf{Comparison Between Indian Work Culture and Japanese Work Culture}\\
  \url{https://pdfcoffee.com/comparison-between-indian-work-\\culture-and-japanese-work-culture-\\with-regards-to-different-companies\\-pdf-free.html}
  
  \item \textbf{India, Japanese Work Culture, and Mental Health} \\
  \url{https://zeromindlab.com/india-japanese-work-culture-and\\-mental-health/}
  
  \item \textbf{Japanese and Indian Work Cultures Are Starkly Different} \\
  \url{https://economictimes.indiatimes.com/japanese-and-indian-work-cultures-are-\\starkly-different-geetanjali-kirloskar/articleshow/45977707.cms}
  
  \item \textbf{5 Ways Japanese Work Culture is Drastically Different from the US} \\
  \url{https://www.businessinsider.in/5-ways-japanese-work-culture-is-\\drastically-different-from-the-us/articleshow/63523612.cms}
  
  \item \textbf{Similarities and Differences Between India and the Middle East (Quora)} \\
  \url{https://www.quora.com/What-are-the-similarities-and-\\differences-between-India-and-the\\-Middle-East}
  
  \item \textbf{Differences Between Arabs and Indians} \\
  \url{http://www.differencebetween.net/miscellaneous/culture-miscellaneous/differences-between-arabs-and-indians/}
  
  \item \textbf{Difference Between Arabs and Indians (Ask Any Difference)} \\
  \url{https://askanydifference.com/difference-between-arabs-and-indians/}
  
  \item \textbf{India's Middle East Strategy} \\
  \url{https://www.csis.org/analysis/indias-middle-east-strategy}
  
  \item \textbf{India and the Middle East: Similarities in Cuisine} \\
  \url{https://en.vogue.me/culture/india-middle-east-cuisine-food-dishes\\-similarities/}
  
  \item \textbf{India and Africa: Similarities and Differences} \\
  \url{https://www.jstor.org/stable/40835868?searchText=&searchUri=&ab_segments=&searchKey=&refreqid=fastly-default%3A10c9bfae536e5ad2f656cebdc14b5c79&seq=5}

  \item \textbf{Cultural Diversity in India and Africa: A Strength, Not a Problem} \\
  \url{https://africaindia.org/cultural-diversity-in-india\\-and-africa-a-strength-not-a-problem/}
  \item \textbf{Japanese Culture: Do's and Don'ts} \
\url{https://expertworldtravel.com/dos-donts-japanese-culture-tips/}

\item \textbf{Japanese Culture: Greetings} \
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-greetings}

\item \textbf{Japanese Culture: Family} \
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-family}

\item \textbf{Japanese Culture: Naming} \
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-naming}

\item \textbf{Japanese Culture: Communication} \
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-communication}

\item \textbf{Japanese Culture: Other Considerations} \
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-other-considerations}

\item \textbf{Japanese Culture: Business Culture} \
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-business-culture}

\item \textbf{Japanese Business Etiquette} \
\url{https://planetdepos.com/trending/content/japanese-business-etiquette}

\item \textbf{Japan Guide: Etiquette and Customs} \
\url{https://www.japan-guide.com/e/e622.html}

\item \textbf{South Korean Culture: Greetings} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-greetings}

\item \textbf{South Korean Culture: Family} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-family}

\item \textbf{South Korean Culture: Naming} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-naming}

\item \textbf{South Korean Culture: Etiquette} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-etiquette}

\item \textbf{South Korean Culture: Do's and Don'ts} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-do-s-and-don-ts}

\item \textbf{South Korean Culture: Communication} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-communication}

\item \textbf{South Korean Culture: Other Considerations} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-other-considerations}

\item \textbf{South Korean Culture: Business Culture} \
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-business-culture}

\item \textbf{Korean Etiquette} \
\url{https://www.90daykorean.com/korean-etiquette/}

\item \textbf{Cramming Korean: Please Take Care of Me} \
\url{https://noonasoverforks.com/2014/09/01/cramming-korean-please-take-care-of-me/}

\item \textbf{How to Greet People in Korea: 2 Steps with Pictures} \
\url{https://medium.com/story-of-eggbun-education/how-to-greet-people-in-korea-2-steps\\-with-pictures-3cc4bd6d25c3}

\item \textbf{Taiwan Etiquette} \
\url{http://www.ediplomat.com/np/cultural_etiquette/ce_tw.htm}

\item \textbf{Culture, Customs, and Etiquette in Taiwan} \
\url{https://www.commisceo-global.com/resources/country-guides/taiwan-guide}

\item \textbf{Taiwanese Culture: Greetings} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-greetings}

\item \textbf{Taiwanese Culture: Family} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-family}

\item \textbf{Taiwanese Culture: Naming} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-naming}

\item \textbf{Taiwanese Culture: Etiquette} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-etiquette}

\item \textbf{Taiwanese Culture: Do's and Don'ts} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-do-s-and-don-ts}

\item \textbf{Taiwanese Culture: Communication} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-communication}

\item \textbf{Taiwanese Culture: Other Considerations} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-other-considerations}

\item \textbf{Taiwanese Culture: Business Culture} \
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-business-culture}
\item \textbf{Arab Academy: Your Guide to Arab Etiquette} \
\url{https://www.arabacademy.com/your-guide-to-arab-etiquette/}

\item \textbf{Etiquette in the Middle East (Wikipedia)} \
\url{https://en.m.wikipedia.org/wiki/Etiquette_in_the_Middle_East}

\item \textbf{Middle East Etiquette Tips} \
\url{https://www.travelawaits.com/2494430/middle-east-etiquette/}

\item \textbf{Etiquette 101: The Do's and Don'ts of Visiting an Arab Home} \
\url{https://theculturetrip.com/middle-east/united-arab-emirates/articles/etiquette-101-the-dos-and-donts\\-of-visiting-an-arab-home/}

\item \textbf{Arabic Customs and Etiquette: What to Consider When in the Middle East} \
\url{https://kaleela.com/en/arabic-customs-and-etiquette-what-to\\-consider-when-in-middle-east}

\item \textbf{Manners in the Middle East (Aramco World)} \
\url{https://archive.aramcoworld.com/issue/196502/manners.in.the.middle.east.html}

\item \textbf{South African Culture: Etiquette} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-etiquette}

\item \textbf{South African Culture: Greetings} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-greetings}

\item \textbf{South African Culture: Naming} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-naming}

\item \textbf{South African Culture: Do's and Don'ts} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-do-s-and-don-ts}

\item \textbf{South African Culture: Communication} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-communication}

\item \textbf{South African Culture: Other Considerations} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-other-\\considerations}

\item \textbf{South African Culture: Business Culture} \
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-business-culture}

\item \textbf{Zimbabwean Culture: Greetings} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-greetings}

\item \textbf{Zimbabwean Culture: Family} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-family}

\item \textbf{Zimbabwean Culture: Naming} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-naming}

\item \textbf{Zimbabwean Culture: Etiquette} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-etiquette}

\item \textbf{Zimbabwean Culture: Do's and Don'ts} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-do-s-and-don-ts}

\item \textbf{Zimbabwean Culture: Communication} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-communication}

\item \textbf{Zimbabwean Culture: Other Considerations} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-other-considerations}

\item \textbf{Zimbabwean Culture: Business Culture} \
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-business-culture}

\item \textbf{Etiquette in Latin America (Wikipedia)} \
\url{https://en.wikipedia.org/wiki/Etiquette_in_Latin_America}

\item \textbf{Business Etiquette in Latin America} \
\url{https://www.jeffreygroup.com/agency-perspectives/business-etiquette-in-latin-america/}

\item \textbf{Cultural Pitfalls to Avoid in Latin America} \
\url{https://www.allianceexperts.com/the-most-important-cultural-pitfalls\\-to-avoid-in-latin-america/}

\item \textbf{The Etiquette of Business in Latin America} \
\url{https://www.languagereach.com/the-etiquette-of-business-in-latin-america/}

\item \textbf{South American Etiquette: How Different Is It?} \
\url{https://thespanishgroup.org/blog/how-different-is-south-american-etiquette\\-from-the-rest-of-the-world/}

\end{itemize}

